Prosperity: Accelerating Spiking Neural Networks via Product Sparsity

Spiking Neural Networks (SNNs) are highly efficient due to their spike-based activation, which inherently produces bit-sparse computation patterns. Existing hardware implementations of SNNs leverage this sparsity pattern to avoid wasteful zero-value computations, yet this approach fails to fully capitalize on the potential efficiency of SNNs. This study introduces a novel sparsity paradigm called Product Sparsity, which leverages combinatorial similarities within matrix multiplication operations to reuse the inner product result and reduce redundant computations. Product Sparsity significantly enhances sparsity in SNNs without compromising the original computation results compared to traditional bit sparsity methods. For instance, in the SpikeBERT SNN model, Product Sparsity achieves a density of only $1.23\%$ and reduces computation by $11\times$, compared to bit sparsity, which has a density of $13.19\%$. To efficiently implement Product Sparsity, we propose Prosperity, an architecture that addresses the challenges of identifying and eliminating redundant computations in real-time. Compared to prior SNN accelerator PTB and the A100 GPU, Prosperity achieves an average speedup of $7.4\times$ and $1.8\times$, respectively, along with energy efficiency improvements of $8.0\times$ and $193\times$, respectively. The code for Prosperity is available at https://github.com/dubcyfor3/Prosperity.

==> content/9transformer.tex <==
\section{Other Designs in \name}

\subsection{Support for Spiking Transformers}
To support the distinctive operations in spiking transformers, we configure the dataflow to reuse the hardware in our PPU. With the cooperation of the SFU, our accelerator is capable of performing various operations in spiking transformers with little overhead, embracing different types of attention, layer normalization, and skip connections.

\subsubsection{Support Attention through PPU}
We consider three canonical types of spiking attention used in different spiking transformer models.

\textbf{Half spiking attention} is proposed by SpikingBERT~\cite{bal2024spikingbert}.
It receives key $K$ and value $V$ of shape $(L,d)$ in spike format in each time step.
The query $Q$ is in floating-point format of shape $(L,d)$ in each time step, as it is directly generated by spiking GeMM in the previous layer, without passing through a spiking neuron.
In each time step, the same computation as vanilla multi-headed attention~\cite{vaswani2017attention} is performed between $Q$, $K$, and $V$.
Therefore, the operation first becomes spike $K$ multiplied by floating-point $Q^T$, yielding a floating-point attention score matrix $S$.
Spike $V^T$ is multiplied with floating-point $S$ after softmax.
These two multiplications are equivalent to spiking GeMM.
Therefore, we load $Q$, $K$, $V$, and $S$ to the correct buffer and reuse the PPU to realize these two multiplications.
For softmax, the sum-up is supported by reusing the PE array in PPU; it works collaboratively with the exponentiate unit, multiplier, and divider in SFU to complete the whole process of softmax.

The result of $V^T \cdot S$ is sent to the spiking neuron array and converted to spikes.
\textbf{Full spiking attention} is proposed by Spikformer~\cite{zhou2022spikformer}.
$Q$, $K$, and $V$ are all in spike form of shape $(L,d)$ in each time step. Multi-headed attention without softmax is performed between $Q$, $K$, and $V$.
We treat the spike $Q$ as a dense floating-point matrix and reuse the PPU for $K \cdot Q^T$.
Elements in the attention score are integers and scaled to floating-point.
We further reuse the PPU for $V^T \cdot S$.
This result is also sent to the spiking neuron array.

\textbf{Linear spiking attention} is proposed by SDT~\cite{yao2024sdt}.
$Q$, $K$, and $V$ are all in spike form of shape $(L,d)$ in each time step.
$Q$ and $K$ first perform a Hadamard product and then sum up in dimension $L$.
The Hadamard product between binary matrices is implemented by bitwise AND in SFU. The AND result is sent to the PE array in PPU for sum-up.
The sum is sent to the spiking neuron array to get a spike vector $S$.
$S$ and $V$ repeat the Hadamard product, sum-up, and are sent to the spiking neuron array.

\name efficiently supports different spiking attention mechanisms due to the disaggregated design of spiking GeMM and spiking neuron operations.
SNN accelerator PTB~\cite{lee2022parallel} embeds the MP update of spiking neurons in the systolic array to implement typical SNN layers.
However, the result of spiking GeMM in attention is not always used to perform MP updates of spiking neurons.
Neuromophic chips Loihi 2~\cite{davies2018loihi} cannot implement spiking attention since it stores static weights in the scratchpad memory of each core but cannot deal with multiplication of two dynamically generated activations.
Moreover, the first two spiking attention mechanisms can benefit from product sparsity to reduce multiple operations.

\subsubsection{Other Operations}
The implementation of layer normalization also reuses the PE array for sum-up. The intermediate result is stored in the output buffer of PPU and transferred to and from SFU for division and multiplication.

Skip connections also exist in some spiking transformers.
The skip connection performed between floating-point input currents~\cite{yao2024sdt} is supported by the PE array in PPU.
The skip connection performed between binary spike matrices~\cite{lv2023spikebert,zhou2022spikformer} may generate non-binary results. To ensure the result is still a binary spike, we modify the addition to bitwise OR, which has been proven to have minor accuracy drop.


